Facilitating Daily Practice in Intangible Cultural Heritage through Virtual Reality: A Case Study of Traditional Chinese Flower Arrangement

The essence of intangible cultural heritage (ICH) lies in the living knowledge and skills passed down through generations. Daily practice plays a vital role in revitalizing ICH by fostering continuous learning and improvement. However, limited resources and accessibility pose significant challenges to sustaining such practice. Virtual reality (VR) has shown promise in supporting extensive skill training. Unlike technical skill training, ICH daily practice prioritizes cultivating a deeper understanding of cultural meanings and values. This study explores VR's potential in facilitating ICH daily practice through a case study of Traditional Chinese Flower Arrangement (TCFA). By investigating TCFA learners' challenges and expectations, we designed and evaluated FloraJing, a VR system enriched with cultural elements to support sustained TCFA practice. Findings reveal that FloraJing promotes progressive reflection, and continuous enhances technical improvement and cultural understanding. We further propose design implications for VR applications aimed at fostering ICH daily practice in both knowledge and skills.

==> Chapters/08Limitation.tex <==

% limitation
% 1. For example, an aspect that remains unclear is why, in the ms, the authors mention that two of them conducted the workshop while they were still learning the craft, despite having experts in the group. Why was not a professional expert directly involved in the research? Wouldn’t that have given an added value? And what type of inaccuracy, or benefits this might bring to the research?




